EM's Convergence in Gaussian Latent Tree Models

We study the optimization landscape of the log-likelihood function and the convergence of the Expectation-Maximization (EM) algorithm in latent Gaussian tree models, i.e. tree-structured Gaussian graphical models whose leaf nodes are observable and non-leaf nodes are unobservable. We show that the unique non-trivial stationary point of the population log-likelihood is its global maximum, and establish that the expectation-maximization algorithm is guaranteed to converge to it in the single latent variable case. Our results for the landscape of the log-likelihood function in general latent tree models provide support for the extensive practical use of maximum likelihood based-methods in this setting. Our results for the EM algorithm extend an emerging line of work on obtaining global convergence guarantees for this celebrated algorithm. We show our results for the non-trivial stationary points of the log-likelihood by arguing that a certain system of polynomial equations obtained from the EM updates has a unique non-trivial solution. The global convergence of the EM algorithm follows by arguing that all trivial fixed points are higher-order saddle points.

==> older.tex <==

\section{Outline}
\begin{itemize}
    \item Definition of the model: Gaussian, structure, covariance and inverse covariance, conditional distribution of $x_i$ and $y$ given $x_1,\dots,x_n$. Notations: nodes $y,x_1,\dots,x_n$, variances $\sigma_y^2$, $\sigma_{x_i}^2$. Covariance matrix $\Sigma$. Inverse covariance $J$, with $J_{x_iy}$ etc. Correlations $\rho_i$. Parameters $\lambda_i$. Vectors $\x$.
    \item EM: for the continuous sample. Define the next iteration given the current iteration. Properties of the next iteration (covariances and variances the same as the mixed distribution). Write explicitly the update rules for $\rho_i$ and covariances. Notations: $\mu^*$, $\mu^t$, $\mu^{t,*}$, $\rho_i^t$, $\rho_i^*$, $\lambda_i^t$ etc.
    \item 
    Outline proof of convergence. Say that we cannot learn the variance of $y$ (look at $\Sigma$ and say that it isn't affected if we change $\sigma_y$). Let's assume that $\sigma_{x_i}^* = \sigma^*_y = 1$. That's because $\sigma^t_{x_i} = \sigma^*_{x_i}$, so the $\sigma_{x_i}$ are going to be correct and it is sufficient to prove convergence on $\rho_i$, And the update on $\rho_i$ is independent of $\sigma_{x_i}$.
    
    We only analyze convergence in terms of $\rho_i$. Since the EM improves in each iteration, the likelihood values converge to something. ....
    
    It is sufficent to show that there's no attractive stationary point other than the true one. Define what is a stationary point, and what equations should be satisfied there. The stationary point is defined as one where the correlations remain the same in the next iteration. 
    
    
    
    Classify the stationary points: with values between $0$ and $1$, at least one value is zero, at least one value is $1$. Say what happens in each of these.
    
    \item Interior:  We show that this means that the likelihood value remains the same. This in turn implies that the variances and covariances of the underlying model remain the same in the new iteration (because otherwise the lower bound would have some increase in likelihood).
    
    \item At $0$: I have a lemma stating that nobody is getting close to $0$.
    
    \item At $1$: not possible for two weights to be one (likelihood is $-\inf$).
    
    One is at $1$: assume wlog that $\rho_1=1$. There is a unique stationary point. We want to understand what happens around this point. 
    \begin{itemize}
        \item There is a second order term that pushes you back, depends only on the distance of $\rho_1$ from $1$.
        \item After one iteration, the errors of the others is same order as $1-\rho_1$. So we can plug it in the formula above to show that we repel from the stationary point.
        \item There is some constant, such that if $\rho_i$ is greater than this constant, than after one iteration it will go back until it goes below it.
    \end{itemize}
\end{itemize}



\section{older - One hidden}

We would like to analyze the EM algorithm for Gaussian graphical models with one hidden variable. In particular, we assume a distribution over one latent variable $y$ and $n$ observed variables $x_1,\dots,x_n$ such that the joint distribution is a jointly Gaussian that is factorized as $\Pr[y,x_1,\dots,x_n] = \Pr[y]\prod_i\Pr[x_i\mid y]$. The algorithm observes $m$ samples of only $\vec x = x_1,\dots,x_n$ and the goal is to recover the original distribution $\mu^*$. Denote by $\mu_{\vec x}$ the marginal distribution of $\mu$ over $\vec x$ and denote by $\mu_{y \mid \vec x}$ the conditional distribution of $y$ given $\vec x$, according to $\mu$.
We abuse notation by letting $\mu$ to also denote the corresponding density function.
Let $\mathcal P$ be the set of all such distributions. Denote by 
We analyze the EM algorithm, that in each iteration $i$, it maintains some distribution $\mu_t \in \mathcal P$, and the next iteration is chosen as
\[
\mu_{t+1} = \max_{\mu \in \mathcal P} \E_{\vec x \sim \mu^*_{\vec x}} \E_{y \sim, \mu^t_{y \mid \vec x}}[\log \mu(\vec x, y)].
\]
Our goal is to prove that $\mu_{t+1}$ converges to $\mu^*$. We will use the following notation: define by
\[
\rho_i(\mu) = \frac{\E_{\vec x,y \sim \mu} x_i y}{\sqrt{\Var_\mu(x_i) \Var_{\mu}(y)}}.
\]
This is the correlation betweein $x_i$ and $y$. Notice that for Gaussian models, we have $\rho_i \in [-1,1]$. We start by assuming that $\rho_i \in[0,1]$ and then argue for negative correlation. Define by $\rho_i^* = \rho_i(\mu^*)$ and $\rho_i^t = \rho_i(\mu^t)$.

We will show that $\rho_i^t$ converge to $\rho_i^*$. For that purpose, let us derive a formula for $\rho_i^{t+1}$ as a function of $\v\rho_i^t = (\rho_1^t,\dots,\rho_n^t)$.
We have the following proposition:
\begin{lemma}
Let $\mu^{t,*}$ denote the joint distribution over $\v x,y$ such that
\[
\mu^{t,*}(\x,y) = \mu^*(\x)\mu^t_{y\mid \v x}(y).
\]
Then,
\[
\v\rho^{t+1} = \v\rho(\mu^{t,*}).
\]
Further, for any $i$, we have that
\[
\E_{\mu^{t+1}}[x_i y] = \E_{\mu^{t,*}}[x_i y], \ \Var_{\mu^{t,*}}[x_i] = \Var_{\mu^{t+1}}[x_i],\ 
\Var_{\mu^{t,*}}[y] = \Var_{\mu^{t+1}}[y]
\]
\end{lemma}
\begin{proof}
Notice that $\mu^{t+1}$ is the MLE over $\mathcal P$ over samples drawn from $\mu^{t,*}$. So, for any $\mu \in \mathcal P$,
\[
\E_{\x,y\sim \mu^{t,*}}\log \mu(\x,y)
= \E_{\x,y\sim \mu^{t,*}}\log\mu(y) \prod_i \mu(x_i\mid y)
= \E_{\x,y\sim \mu^{t,*}}\log\mu(y) + \sum_i \E_{\x,y\sim \mu^{t,*}}\log\mu(x_i\mid y).
\]
We can find a distribution that maximizes all of the terms in the right hand side (separately, not only their sum). By Gibbs inequality,
\[
\E_{\x,y\sim \mu^{t,*}}\log\mu(y)
\]
is maximized by any distribution that has the same marginal as $y$. Similarly, $\E_{\x,y\sim \mu^{t,*}}\log\mu(x_i\mid y)$ is maximized by any distribution that has the same conditional distribution of $x_i$ given $y$ as $\mu^{t,*}$. In particular, if we choose a distribution $\mu'$ that has the same marginal as $y$ and the same conditionals of $x_i$ given $y$, then it maximizes all the terms in the right hand side above, and particularly, it maximizes their sum. Which implies that $\mu' = \mu^{t+1}$. Uniqueness follows from the fact that the distributions in $\mathcal P$ factorize as $\mu(y) \prod_i \mu(x_i \mid y)$, so any two such distributions that match $\mu(y)$ and $\mu(x_i\mid y)$ for all $i$ must be identical.

Notice that
\[
\mu^{t+1}(x_i,y) = \mu^{t+1}(y) \mu^{t+1}(x_i\mid y) =  \mu^{t,
*}(y) \mu^{t,*}(x_i\mid y) = \mu^{t,*}(x_i,y),
\]
in particular, the variances of $x_i,y$ and $\Cov(x_i,y)$ should be identical in the two distributions as required. Consequently, the correlations $\rho_i$ are also identical.
\end{proof}

We will assume that $\rho^*_i \in (0,1)$ for all $i$. We would like to study the stationary points of the EM iterations, namely, distributions $\mu$ such that $\mu^{t+1} = \mu^t$ whenever $\mu^t = \mu$. There can be three types of such distributions:
\begin{itemize}
    \item Distributions such that $\rho_i = 0$ for some $i$.
    \item Distributions such that $\rho_i \in (0,1)$ for all $i$.
    \item Distributions such that $\rho_i > 0$ for all $i$ and there exists some $j$ such that $\rho_j = 1$.
\end{itemize}

\paragraph{Distributions such that $\rho_i \in (0,1)$ for all $i$.}
We will start with the second type of distributions, and show that there is only one stationary distribution. In particular, since $\mu^*$ is stationary, we get that there is no other such distribution. We have that a stationary distribution $\mu^t$ must satisfy
\[
\E_{\mu^{t}} [x_i y] = \E_{\mu^{t+1}}[x_i y] = \E_{\mu^{t,*}}[x_i y].
\]
Let us analyze this in more depth. We note that given fixed $\x$, $\E_{\mu^t}[y\mid x]$ is a linear combination of $x$. This is due to the fact that the conditional expectation of one variable given the others is always linear in jointly Gaussian distributions. Let $\lambda_1,\dots,\lambda_n$ denote the coefficients, namely,
\[
\E_{\mu_t}[y\mid x] = \sum_i \lambda_i x_i.
\]
We derive that
\[
\E_{\mu_t}[x_i y] = \E_{\mu^t_{\x}}[\E_{\mu^t_{y\mid \x}}[x_i y]]
= \E_{\mu^t_{\x}}[x_i\sum_i \lambda_j x_j]
= \sum_{j} \lambda_j \E_{\mu^t_{\x}}[x_i x_j].
\]
Similarly,
\[
\E_{\mu^{t,*}}[x_i y]
= \E_{\mu^*_{\x}}[\E_{\mu^t_{y\mid \x}}[x_i y]]
= \E_{\mu^*_{\x}}[x_i\sum_i \lambda_j x_j]
= \sum_{j} \lambda_j \E_{\mu^*_{\x}}[x_i x_j].
\]
We use the following known fact:
\begin{lemma}
Let $\mu\in \mathcal{P}$, then for any $i \ne j$,
\[
\frac{\E_{\mu}[x_i x_j]}{\sqrt{\Var_\mu(x_i)\Var_\mu(x_j)}}
= \rho_i(\mu)\rho_j(\mu).
\]
\end{lemma}
\begin{proof}
.
\end{proof}
Since $\E_{\mu^t}[x_i y] = \E_{\mu^{t,*}}[x_i y]$, we derive that
\[
\sum_j  \lambda_j \E_{\mu^t_{\x}}[x_i x_j]
= \sum_j \lambda_j \E_{\mu^*_{\x}}[x_i x_j].
\]
By Lemma..., we have that
\[
\E_{\mu^t}[x_i^2] = \E_{\mu^{t+1}}[x_i^2]
= \E_{\mu^{t,*}}[x_i^2]
= \E_{\mu^*}[x_i^2]\enspace.
\]
Hence, we can subtract this from both sides of the equation above and derive that
\[
\sum_{j \ne i} \lambda_j \E_{\mu^t_{\x}}[x_i x_j]
= \sum_{j \ne i} \lambda_j \E_{\mu^*_{\x}}[x_i x_j].
\]
Substituting using Lemma..., we derive that
\[
\sum_{j \ne i} \lambda_j \rho^t_i \rho^t_j
= \sum_{j \ne i} \lambda_j \rho^*_i \rho^*_j.
\]
Recall that $\lambda_j$ are the parameters corresponding the conditional distribution of $y$ given $x$ according to $\rho^t$. The following follows from a simple calculation:
\begin{lemma}
Assuming that $\rho^t_i > 0$, then $\lambda_i > 0$.
\end{lemma}
\begin{proof}
.
\end{proof}
Since we assumed that $\rho_i^t>0$ for all $i$ it implies that $\lambda_i>0$. Then, the above equations can be multiplies by $\lambda_i$, to get that for all $i$,
\[
\sum_{j \ne i} \lambda_i\lambda_j \rho^t_i \rho^t_j
= \sum_{j \ne i} \lambda_i\lambda_j \rho^*_i \rho^*_j\enspace.
\]
Substitute $\rho^t_i \lambda_i = u^t_i$ and $\rho^*_j \lambda_j = u^*_j$, we derive that
\[
\sum_{j \ne i} u^t_iu^t_j
= \sum_{j \ne i} u^*_iu^*_j\enspace.
\]
We would like to show that there are no two distinct vectors, $\v u^*$ and $\v u^t$, of positive entries, that satisfy the above equations. For this purpose, we have the following lemma:
\begin{lemma}
Let $p_1,\dots,p_n$ a collection of quadratic polynomials over $x_1,\dots,x_n$. If there are two distinct vectors, $\v u$ and $\v u^t$ such that $p_j(\v u) = p_j(\v u')$ for all $j$, then, the Jacobian matrix of $\v p$ computed at $(\v u+\v u')/2$, $J^{\v p}((\v u + \v u')/2)$, is singular, where
\[
J^{\v p}_{i,j}(\v v)
= \frac{dp_i(\v v)}{dv_j}.
\]
\end{lemma}
\begin{proof}
Look at the path $\gamma \colon [0,1]\to \mathbb{R}^n$ defined by $\gamma(s) = s \v u + (1-s) \v u'$. Then, $p_i(\gamma(s))$ is a quadratic polynomial in $s$, that satisfies $p_i(\gamma(0)) = p_i(\gamma(1))$. Therefore, $1/2$ is a point, hence
\[
0 = \frac{d}{ds} p_i(\gamma(s))
= \sum_j \frac{d p_i}{dv_j} \frac{d\gamma_j}{ds}
= \sum_j \frac{d p_i}{dv_j}\bigg|_{\v v = \gamma(1/2)} (\v u' - \v u)
= (J^{\v p}(\v\gamma(1/2))) (\v u'-\v u)
= (J^{\v p}((\v u + \v u')/2)) (\v u'-\v u),
\]
hence $J^{\v p}((\v u + \v u')/2)$ is singular.
\end{proof}
To complete the proof, let us substitute $p_i(\v u) = \sum_{j\ne i} u_i u_j$ and that Jacobian is
\[
J_{i,j}^{\v p}(\v u) = \begin{cases}
\sum_{k \ne i} u_k & i = j \\
u_i & i \ne j
\end{cases}\enspace.
\]
We would like to substitute $\v u = \v u^t$ and $\v u' = \v u^*$, and notice that all the entries of both vectors are positive, hence, all the entries of $(\v u + \v u')/2$ are positive, which implies that it is sufficient to look at the Jacobian in points where all $u_i$ are positive. For that, we have the following lemma:
\begin{lemma}
Let $\v \theta$ be a vector with $\theta_i > 0$ for all $i$, and let $J$ be the matrix such that
\[
J_{ij} = \begin{cases}
\sum_{k \ne i} \theta_k & i = j\\
u_i & i \ne j
\end{cases}.
\]
Then, $J$ is non-singular.
\end{lemma}
\begin{proof}
We would like to show that there is no nontrivial solution $a$ for $Ja=0$. We have
\[
(Ja)_i = \sum_{j \ne i} a_j \theta_j  + a_i (\sum_{j \ne i} \theta_j)
= \sum_j a_j \theta_j + a_i(\sum_j \theta_j - 2\theta_i).
\]
Substitute $s = \sum_j \theta_j$ and $u = \sum_j a_j \theta_j$, we have
\[
(Ja)_i = u + a_i (s-2\theta_i).
\]
To solve the system of equations $Ja=0$, we assume without loss of generality that $\theta_1 = \max_j \theta_j$
and divide into cases according to $\theta_1$. First, assume that $\theta_1 < s/2$. Then,
\begin{equation}\label{eq:ai-equation-raw}
(Ja)_i = u + a_i(s-2\theta_i) = 0
\end{equation}
implies
\[
a_i = \frac{-u}{s-2\theta_i}.
\]
The equation $\sum_i \theta_i a_i = u$ implies
\begin{equation}\label{eq:with-u}
\sum_i \theta_i a_i = \sum_i \frac{-u \theta_i}{s-2\theta_i} = u.
\end{equation}
Notice that $u \ne 0$. Assume towards contradiction that $u = 0$. Then, we have
\[
0 = a_i (s- 2 \theta_i).
\]
Dividing by $s- 2 \theta_i$ we get $a_i = 0$ for all $i$. Since we look for nontrivial solutions $a$ to $Ja=0$, we assume that $a\ne 0$ which implies that $u \ne 0$.
Dividing \eqref{eq:with-u} by $u$ we get
\begin{equation}\label{eq:theta1small}
\sum_i \frac{-\theta_i}{s-2\theta_i} = 1.
\end{equation}
By the assumption $\theta_1 < s/2$ we have $s-2\theta_i \ge s-2\theta_1 > 0$. In particular, the left hand side of \eqref{eq:theta1small} is negative while the right hand side is positive, hence there is no solution! Next, assume that $\theta_1 > s/2$. In this case, we have $\theta_i < s/2$ for all $i\ge 2$, since $\sum_i \theta_i = s$. Here, \eqref{eq:theta1small} is still valid, and is equivalent to
\[
\frac{\theta_1}{2\theta_1-s} - 1 = \sum_{i>1} \frac{\theta_i}{s-2\theta_i},
\]
which is equivalent to
\[
\frac{s - \theta_1}{2\theta_1-s} = \sum_{i>1} \frac{\theta_i}{s-2\theta_i}\enspace.
\]
Here, we will show that the left hand side is strictly greater than the right hand side, which implies that there is no equality. First, notice that for any $i \ge 2$, $2\theta_1 - s < s - 2 \theta_i$. Indeed, this follows from $s = \sum_j \theta_j > \theta_1 + \theta_i$, since all $\theta_j$ are positive and $n\ge 3$. We derive that
\[
\frac{s - \theta_1}{2\theta_1-s} =
\sum_{i \ge 2} \frac{\theta_i}{2\theta_1-s} >
\sum_{i \ge 2} \frac{\theta_i}{s - 2\theta_i}\enspace,
\]
which arrives at a contradiction. Lastly, assume that $\theta_1 = s/2$. Since $s = \sum_{i=1}^n \theta_i$ and $n \ge 3$, then for all $i\ge 2$ we have $\theta_i < s/2$. Recall \eqref{eq:ai-equation-raw} which states that 
\[
0 = (Ja)_i = u + a_i(s-2\theta_i).
\]
Applying with $i=1$ we obtain
\[
u = 0.
\]
For all $i \ge 2$ we have
\[
a_i(s - 2 \theta_i) = 0
\]
which implies that $a_i = 0$ for $i \ge 2$. By definition of $u$ and by the computations above,
\[
0 = u = \sum_i a_i \theta_i = a_1 \theta_1.
\]
Since $\theta_1 > 0$ we have
\[
a_1 = 0.
\]
We conclude that $a_i = 0$ for all $i$ which implies that there is no nontrivial solution for $Ja=0$, as required.
\end{proof}

\section{others}


\begin{lemma}
	We assume that for all $i$, $A \le \rho^*_i \le B$. If for some $i$, $\rho_i^t \le \min(A^2/2B,A/(B/A+2B))$. Then $ \rho^{t+1}_i \ge \rho_i^t$.
\end{lemma}
\begin{proof}
	Denote $\rho_j = \rho_j^t$, $\rho_j' = \rho_j^{t+1}$ and $\Delta_{ij} = \Delta_{ij}^t$.
	Notice that $\rho_i \rho_j \le \rho_i B \le A^2/2 \le \rho^*_i \rho^*_j/2$, which implies that $\Delta_{ij} \ge \rho^*_i \rho^*_j/2$. 
	Further, $\Delta_{jk} \le \rho^*_i \rho^*_j$ for all $j,k$. Then, from Lemma~\ref{lem:update},
	\[
	\rho'_i \ge \frac{\rho_i + \sum_{j\ne i} \lambda_j \rho^*_i \rho^*_j/2}{\sqrt{1 + \sum_{j, k \colon j\ne k} \rho^*_j\rho^*_k \lambda_j \lambda_k}}
	\ge \frac{\rho_i + \sum_{j\ne i} \lambda_j \rho^*_i \rho^*_j/2}{1 + \sum_{j, k \colon j\ne k} \rho^*_j\rho^*_k \lambda_j \lambda_k}.
	\]
	Notice that $\sum_j \rho_j \lambda_j \le 1$, hence,
	\[
	\sum_j \rho^*_j \lambda_j = \sum_j \frac{\rho^*_j}{\rho_j} \rho_j \lambda_j
	\le \frac{B}{A} \sum_j \rho_j \lambda_j
	\le \frac{B}{A}.
	\]
	Further, 
	\[
	\sum_{j \ne k} \rho^*_j \lambda_j \rho^*_k \lambda_k
	\le \left(\sum_{j\ne i} \rho^*_j \lambda_j\right)^2 + 2 \rho^*_i \sum_{j\ne i} \rho^*_j \lambda_j \le
	\left(\frac{B}{A} + 2\rho^*_i \right) \sum_{j \ne i} \rho^*_j \lambda_j.
	\]
	Denote $K = \sum_{j\ne i} \rho^*_j \lambda_j$. Then,
	\[
	\rho'_i \ge \frac{\rho_i + \rho^*_i K}{1+(B/A+2\rho^*_i)K}
	= \rho_i \frac{1 + \frac{\rho^*_i}{\rho_i} K}{1+(B/A+2\rho^*_i)K}.
	\]
	It suffices to show that $\rho^*_i/\rho_i \ge B/A+2\rho^*$. Indeed,
	\[
	\frac{\rho^*_i}{\rho_i} \ge \frac{A}{\rho_i}
	\ge \frac{B}{A}+2B
	\ge \frac{B}{A}+2\rho^*_i,
	\]
	as required.
\end{proof}


\begin{proof}
\yuval{to delete}
Notice that $\mu^{t+1}$ is the MLE over $\mathcal P$, given samples drawn from $\mu^{t,*}$. Hence, for any $\mu \in \mathcal P$,
\[
\E_{\x,y\sim \mu^{t,*}}\log \mu(\x,y)
= \E_{\x,y\sim \mu^{t,*}}\log\mu(y) \prod_i \mu(x_i\mid y)
= \E_{\x,y\sim \mu^{t,*}}\log\mu(y) + \sum_i \E_{\x,y\sim \mu^{t,*}}\log\mu(x_i\mid y).
\]
We can find a distribution that maximizes all of the terms in the right hand side (separately, not only their sum). By Gibbs inequality,
\[
\E_{\x,y\sim \mu^{t,*}}\log\mu(y)
\]
is maximized by any distribution that has the same marginal as $y$. Similarly, $\E_{\x,y\sim \mu^{t,*}}\log\mu(x_i\mid y)$ is maximized by any distribution that has the same conditional distribution of $x_i$ given $y$ as $\mu^{t,*}$. In particular, if we choose a distribution $\mu'$ that has the same marginal as $y$ and the same conditionals of $x_i$ given $y$, then it maximizes all the terms in the right hand side above, and particularly, it maximizes their sum. Which implies that $\mu' = \mu^{t+1}$. Uniqueness follows from the fact that the distributions in $\mathcal P$ factorize as $\mu(y) \prod_i \mu(x_i \mid y)$, so any two such distributions that match $\mu(y)$ and $\mu(x_i\mid y)$ for all $i$ must be identical.

Notice that
\[
\mu^{t+1}(x_i,y) = \mu^{t+1}(y) \mu^{t+1}(x_i\mid y) =  \mu^{t,
*}(y) \mu^{t,*}(x_i\mid y) = \mu^{t,*}(x_i,y),
\]
in particular, the variances of $x_i,y$ and $\Cov(x_i,y)$ should be identical in the two distributions as required. Consequently, the correlations $\rho_i$ are also identical.
\end{proof}

